VLA-ULAP: Interleaving Cloud VLA Calls with Ultra-Lightweight Local Action Prediction at the Edge

Billion-parameter vision-language-action (VLA) policies run either onboard, consuming substantial power, or on remote servers, adding communication latency. To address these drawbacks and better balance latency and onboard energy consumption, we propose VLA-ULAP. It partitions inference across decision times, interleaving remote VLA calls with predictions from an Ultra-Lightweight Local Action Predictor (ULAP). A single ULAP has $\sim$7.4M parameters including the frozen vision encoder. It combines current views, proprioception, and executed action history to predict chunks in one pass. Trained independently, it requires no VLA hidden states, online verification, or server round trips. On Jetson Orin Nano, ULAP takes 20.7 ms and 0.122 J of idle-subtracted energy per inference, versus 289.3 ms and 40.46 J for GR00T on RTX A6000. Across four simulated base-policy/benchmark pairs, VLA-ULAP removes 45.3-77.3% of VLA calls while retaining 95.0-98.5% of baseline success rates at selected operating points. On VLA-JEPA, VLA-ULAP also surpasses local acceleration alternatives, using an estimated 49.4% less inference time and 51.5% less GPU energy per successful episode than ACT, and 77.5% less time and 80.7% less energy than SP-VLA at higher success rates. In physical SO-101 trials, it similarly removes 70.3-71.9% of VLA calls without observed success-rate loss at seen or held-out placements. Measured device costs imply 64.6-66.4% less inference time and 70.1-71.7% less idle-subtracted energy per successful episode at these call counts. Beyond these savings, faster responses help VLA-ULAP exceed $\pi_{0.5}$'s success rate by 11.0 and 15.5 percentage points (pp) on two tasks in latency-aware LIBERO-Safety simulation while approximately halving VLA calls.

==> figures/fig_ulap_deployment_baselines.tex <==
% Block 1: two conventional deployments, identical decision granularity.
\node[anchor=north west,inner sep=0pt] (remoteTitle) at (0,0)
  {\textbf{(a) Remote-only}};
\node[anchor=north west,inner sep=0pt] (onboardTitle) at (205,0)
  {\textbf{(b) On-board GPU}};
\draw[mPanelE,line width=.65pt] (195,-3) -- (195,-78);
\node[inner sep=0pt] (remoteServer) at (26,-35)
  {\includegraphics[width=33pt]{figures/assets/ulap_deployment_generated_2026-09-15/server.png}};
\node[inner sep=0pt] (remoteRobot) at (157,-37)
  {\includegraphics[width=46pt]{figures/assets/ulap_deployment_generated_2026-09-15/robot.png}};
\node[anchor=north,inner sep=0pt] at (26,-55) {VLA / GPU};
\node[anchor=north,inner sep=0pt] at (157,-59) {Robot};
% Same simple cloud-node convention as the professor's PowerPoint reference.
\coordinate (networkMid) at ($(remoteServer.east)!0.5!(remoteRobot.west)$);
\node[udnetwork] (network) at (networkMid) {Network};
\draw[marr,<->] (remoteServer.east |- network.center) -- (network.west);
\draw[marr,<->] (network.east) -- (remoteRobot.west |- network.center);
\node[inner sep=0pt,align=center] at (network.center |- 94,-56)
  {\DeployNetworkScale\ / \DeployCommEnergyScale};
\node[anchor=north,inner sep=0pt,text=uDrawback] (remoteDrawback) at (101,-68)
  {\textbf{Added network delay / energy}};
\udface{([xshift=-7pt,yshift=-3pt]remoteDrawback.north west)}{uDrawback}{-1}
% A separate GPU illustration points to its mounting location on the robot.
\node[inner sep=0pt] (onboardGPU) at (241,-39)
  {\includegraphics[width=53pt]{figures/assets/ulap_deployment_generated_2026-09-15/gpu.png}};
\node[inner sep=0pt] (onboardRobot) at (360,-37)
  {\includegraphics[width=48pt]{figures/assets/ulap_deployment_generated_2026-09-15/robot.png}};
\node[anchor=south,inner sep=0pt] at (241,-17) {\textbf{Full VLA}};
\node[anchor=north,inner sep=0pt] at (241,-61) {100s of W};
\node[anchor=north,inner sep=0pt] at (360,-61) {Robot};
\coordinate (onboardMount) at ([xshift=-3pt,yshift=-12pt]onboardRobot.center);
\draw[marr] (onboardGPU.east) -- (308,-39) |- (onboardMount);
\node[inner sep=0pt] at (300,-25) {Mounted on robot};
\node[anchor=north,inner sep=0pt,text=uDrawback] (onboardDrawback) at (300,-68)
  {\textbf{High onboard battery drain}};
\udface{([xshift=-7pt,yshift=-3pt]onboardDrawback.north west)}{uDrawback}{-1}
\node[anchor=north,inner sep=0pt,text=uDrawback] (sharedDrawback) at (200.5,-80)
  {\textbf{Both: latency-onboard-energy trade-off}};
\udface{([xshift=-7pt,yshift=-3pt]sharedDrawback.north west)}{uDrawback}{-1}


==> figures/fig_ulap_deployment_benefits.tex <==
% Block 3: five zero-based comparisons, grouped by the three deployment benefits.
% Source calculations: scripts/prepare_figure1_redesign.py and evidence.json.
% Compact vertical pair: x, title, baseline, local/hybrid, scale, labels, reduction.
\providecommand{\benefitpair}[8]{%
  \begin{scope}[shift={(#1,-28)}]
  \node[anchor=north,inner sep=0pt] at (31,0) {#2};
  \fill[mAuxE] (10,-42) rectangle ++(12,{25*(#3/#5)});
  \fill[uOutputE] (37,-42) rectangle ++(12,{25*(#4/#5)});
  \node[anchor=south,inner sep=0pt] at (16,{-40+25*(#3/#5)}) {#3};
  \node[anchor=south,inner sep=0pt] at (43,{-40+25*(#4/#5)}) {#4};
  \draw[mLine,line width=.5pt] (7,-42) -- (56,-42);
  \node[anchor=east,inner sep=0pt,text=mAuxE] at (4,-42) {0};
  \node[anchor=north,inner sep=0pt] at (16,-45) {#6};
  \node[anchor=north,inner sep=0pt] at (43,-45) {#7};
  \node[anchor=north,inner sep=0pt,text=uOutputE] at (31,-57)
    {\textbf{#8\% less}};
  \end{scope}%
}
\draw[mPanelE,line width=.65pt] (0,-228) -- (391,-228);
\node[udheading,anchor=west,fill=white,inner xsep=0pt,inner ysep=2pt] at (0,-228)
  {Benefits\quad};
\foreach \x in {130,261} {\draw[mPanelE,line width=.5pt] (\x,-239) -- (\x,-344);}
\begin{scope}[shift={(0,-239)}]
\node[anchor=north west,inner sep=0pt] at (0,0) {\textbf{1 More responsive control}};
\node[anchor=north west,inner sep=0pt,text=mAuxE] at (0,-13) {LIBERO-Safety: 2-task mean};
\node[anchor=north west,inner sep=0pt] at (0,-26) {Success rate (\%)};
\node[anchor=east,inner sep=0pt] at (28,-49) {$\pi_{0.5}$};
\node[anchor=east,inner sep=0pt] at (28,-66) {Ours};
\fill[mAuxE] (35,-45) rectangle ++({66*\FigDynBase/100},-8);
\fill[uOutputE] (35,-62) rectangle ++({66*\FigDynOurs/100},-8);
\node[anchor=west,inner sep=0pt] at ({38+66*\FigDynBase/100},-49) {\FigDynBase};
\node[anchor=west,inner sep=0pt] at ({38+66*\FigDynOurs/100},-66) {\FigDynOurs};
\draw[mLine,line width=.5pt] (35,-44) -- (35,-71);
\node[anchor=north,inner sep=0pt,text=mAuxE] at (35,-73) {0};
\node[anchor=north west,inner sep=0pt,text=uOutputE] at (0,-84)
  {\textbf{+\FigDynGain~pp}};
\node[anchor=north west,inner sep=0pt,text=mStaE,align=left] at (12,-97)
  {\textbf{Better success in}\\\textbf{changing scenes}};
\udface{(4,-101)}{mStaE}{1}
\end{scope}
\begin{scope}[shift={(136,-239)}]
\node[anchor=north west,inner sep=0pt] at (0,0) {\textbf{2 Lower total inference cost}};
\node[anchor=north west,inner sep=0pt,text=mAuxE,align=left,font=\sffamily\fontsize{7}{8}\selectfont] at (0,-11)
  {SO-101:\\pick-and-place glue-stick};
\benefitpair{0}{Device energy (J)}{\FigEnergyBase}{\FigEnergyOurs}{1000}{GR00T}{Ours}{\FigEnergyGain}
\benefitpair{63}{Inference (s)}{\FigTimeBase}{\FigTimeOurs}{6}{GR00T}{Ours}{\FigTimeGain}
\end{scope}
\begin{scope}[shift={(267,-239)}]
\node[anchor=north west,inner sep=0pt] at (0,0) {\textbf{3 Affordable, low-power edge}};
\node[anchor=north west,inner sep=0pt,text=mAuxE,align=left,font=\sffamily\fontsize{7}{8}\selectfont] at (0,-11)
  {GR00T on A6000\\Ours on Jetson Orin Nano};
\benefitpair{0}{Energy / call (J)}{\FigVlaJ}{\FigUlapJ}{55}{GR00T}{Ours}{\FigPerEnergyGain}
\benefitpair{63}{Time / call (ms)}{\FigVlaMs}{\FigUlapMs}{300}{GR00T}{Ours}{\FigPerTimeGain}
\node[anchor=north west,inner sep=0pt,text=mStaE,align=left] at (12,-97)
  {\textbf{Longer battery life,}\\\textbf{scalable fleets}};
\udface{(4,-101)}{mStaE}{1}
\end{scope}


==> figures/fig_ulap_deployment_hybrid.tex <==
% Block 2: one local decision loop, with a scheduled cloud or edge branch.
\begin{scope}[yshift=-4pt]
\draw[mPanelE,line width=.65pt] (0,-86) -- (391,-86);
\node[anchor=north west,inner sep=0pt,text=uOutputE] (hybridTitle) at (0,-95)
  {\textbf{(c) VLA-ULAP: Mixed Cloud + Edge inference}};
\node[udserver,minimum width=116pt,minimum height=46pt] (cloudVLA) at (62,-143) {};
\node[inner sep=0pt] (cloudArt) at ([xshift=-38pt]cloudVLA.center)
  {\includegraphics[width=30pt]{figures/assets/ulap_deployment_generated_2026-09-15/server.png}};
\node[align=center,inner sep=0pt] at ([xshift=15pt]cloudVLA.center)
  {\textbf{Shared VLA server}\\GR00T N1.7 on A6000\\\FigVlaMs\,ms / \FigVlaJ\,J};
\node[udbox,minimum width=85pt,minimum height=20pt] (route) at (224,-137)
  {\textbf{Fixed scheduler}};
\node[udedge,minimum width=116pt,minimum height=39pt] (localULAP) at (224,-180) {};
\node[inner sep=0pt] at ([xshift=-43pt]localULAP.center)
  {\includegraphics[width=26pt]{figures/assets/ulap_deployment_generated_2026-09-15/edge.png}};
\node[inner sep=0pt,align=center] at ([xshift=13pt]localULAP.center)
  {\textbf{Local ULAP}\\Jetson Orin Nano\\\FigUlapMs\,ms / \FigUlapJ\,J};
\node[inner sep=0pt] (hybridRobot) at (360,-153)
  {\includegraphics[width=51pt]{figures/assets/ulap_deployment_generated_2026-09-15/robot.png}};
\node[anchor=north,inner sep=0pt] at ([yshift=-1pt]hybridRobot.south) {Robot};
% Every decision observes the robot again before selecting a compute branch.
\draw[marr] (hybridRobot.north) -- ++(0,13pt) -| (route.north);
\node[anchor=south east,inner sep=0pt] at (391,-112)
  {Fresh observations + state + action history};
\draw[udremote] (route.west) -- (cloudVLA.east |- route.west)
  node[midway,above=3pt,inner sep=0pt] {Remote};
\draw[udflow] (route.south) -- (localULAP.north)
  node[midway,right=3pt,inner sep=0pt] {Local};
\coordinate (actionJoin) at (316,-180);
\draw[udremote] ([yshift=-12pt]cloudVLA.east) -- ++(12pt,0) |- (316,-211) -- (actionJoin);
\draw[udflow] (localULAP.east) -- (actionJoin);
\fill[mLine] (actionJoin) circle (1.2pt);
\draw[marr] (actionJoin) |- (hybridRobot.west)
  node[pos=.35,left=3pt,align=right,inner sep=0pt] {Selected\\actions};
% Same sharing relationship for both additional conceptual fleet clients.
\node[inner sep=0pt] (fleetA) at (29,-190)
  {\includegraphics[width=26pt]{figures/assets/ulap_deployment_generated_2026-09-15/robot.png}};
\node[inner sep=0pt] (fleetB) at (92,-190)
  {\includegraphics[width=26pt]{figures/assets/ulap_deployment_generated_2026-09-15/robot.png}};
\draw[udremote,<->] (cloudVLA.south -| fleetA.north) -- (fleetA.north);
\draw[udremote,<->] (cloudVLA.south -| fleetB.north) -- (fleetB.north);
\node[inner sep=0pt,anchor=north] at (60,-208) {Other robots + ULAP};
\end{scope}


==> figures/figure1_result_macros.tex <==
% Generated by scripts/prepare_figure1_redesign.py; see analysis/figure1_redesign_2026-09-15/evidence.json.
\providecommand{\FigDynBase}{63.75}%
\providecommand{\FigDynOurs}{77.00}%
\providecommand{\FigDynGain}{13.25}%
\providecommand{\FigEnergyBase}{769}%
\providecommand{\FigEnergyOurs}{218}%
\providecommand{\FigEnergyGain}{71.7}%
\providecommand{\FigTimeBase}{5.50}%
\providecommand{\FigTimeOurs}{1.84}%
\providecommand{\FigTimeGain}{66.4}%
\providecommand{\FigPerTimeGain}{92.8}%
\providecommand{\FigPerEnergyGain}{99.7}%
\providecommand{\FigVlaMs}{289.3}%
\providecommand{\FigUlapMs}{20.7}%
\providecommand{\FigVlaJ}{40.46}%
\providecommand{\FigUlapJ}{0.122}%


==> result_layout.tex <==
% Paired related plots, each with its own below-figure caption.
% Narrative stays in the section flow, never inside a floating figure.
\makeatletter
% Semantic paragraph continuation beside an illustration. No fixed heights,
% page numbers, line counts or manual page breaks; widths follow the text area.
\newcommand{\resultbeside}[2]{%
  \par\noindent
  \begin{minipage}[t]{.52\linewidth}
    \vspace{0pt}\centering\def\@captype{figure}#1
  \end{minipage}\hfill
  \begin{minipage}[t]{\dimexpr.48\linewidth-1em\relax}
    \vspace{0pt}#2
  \end{minipage}\par
}
% Crop only blank PDF margins: plots remain at native scale and font size.
\newcommand{\resultgraphic}[1]{\includegraphics[trim=0 3bp 0 3bp,clip]{#1}}
\newcommand{\resultsection}[6]{%
  \par\noindent\begin{minipage}{\linewidth}
  \subsection{#1}\label{#2}
  \noindent\begin{minipage}[t]{2.85in}
    \vspace{0pt}\centering\resultgraphic{#3}\par
    \def\@captype{figure}\caption{#4}\label{#5}
  \end{minipage}\hfill
  \begin{minipage}[t]{\dimexpr\linewidth-2.85in-1em\relax}
    \vspace{0pt}\setlength{\parskip}{6pt}#6
  \end{minipage}
  \end{minipage}\par\addvspace{4pt}%
}
\newcommand{\resultpanel}[3]{%
  \begin{minipage}[t]{.49\linewidth}
    \vspace{0pt}\centering
    \resultgraphic{#1}\par
    \caption{#2}\label{#3}
  \end{minipage}%
}
% Unnumbered model/benchmark heading within a shared results subsection.
\newcommand{\resultparagraph}[6]{%
  \par\noindent\begin{minipage}{\linewidth}
  \noindent\begin{minipage}[t]{2.85in}
    \vspace{0pt}\centering\resultgraphic{#3}\par
    \def\@captype{figure}\caption{#4}\label{#5}
  \end{minipage}\hfill
  \begin{minipage}[t]{\dimexpr\linewidth-2.85in-1em\relax}
    \vspace{0pt}\setlength{\parskip}{6pt}\textbf{#1.} #6
  \end{minipage}
  \end{minipage}\par\addvspace{4pt}%
}
\makeatother

